Magic-State Functional Units: Mapping and Scheduling Multi-Level Distillation Circuits for Fault-Tolerant Quantum Architectures

Quantum computers have recently made great strides and are on a long-term path towards useful fault-tolerant computation. A dominant overhead in fault-tolerant quantum computation is the production of high-fidelity encoded qubits, called magic states, which enable reliable error-corrected computation. We present the first detailed designs of hardware functional units that implement space-time optimized magic-state factories for surface code error-corrected machines. Interactions among distant qubits require surface code braids (physical pathways on chip) which must be routed. Magic-state factories are circuits comprised of a complex set of braids that is more difficult to route than quantum circuits considered in previous work [1]. This paper explores the impact of scheduling techniques, such as gate reordering and qubit renaming, and we propose two novel mapping techniques: braid repulsion and dipole moment braid rotation. We combine these techniques with graph partitioning and community detection algorithms, and further introduce a stitching algorithm for mapping subgraphs onto a physical machine. Our results show a factor of 5.64 reduction in space-time volume compared to the best-known previous designs for magic-state factories.

==> old/future.tex <==
\section{Future Work}\label{sec:future}
\subsection{Comparing Distributed Factory Topologies}\label{subsec:arch}
While dividing single factories comes with many benefits, it also raises an implementation question. Choosing an optimal layout for these many factories is potentially very difficult, and requires an ability to estimate the overheads associated with different layouts. Using architectural simulation tools and adapted network simulation mechanisms, we evaluated two distinct architectures: Peripheral and Mesh placement. Peripheral placement refers to placement of factories around the edge of a computational fabric, while Mesh placement refers to embedding the factories within the fabric itself. 




==> old/intro.tex <==
\section{Introduction}\label{sec:Introduction}

 Quantum computation promises to provide computational power required to solve classically intractable problems, and have significant impact in materials science, quantum chemistry, cryptography, communication, and many other fields. Due to the intrinsic fragility of quantum states, quantum error correction is required to ensure that full length quantum programs can execute with high probability of succeeding. The leading conception for implementation of such error correction is surface code \cite{FowlerSurface}, where the overhead appears to be minimal in terms of both fabrication complexity and classical computation intensity required to perform decoding. With typical surface code implementations, universal quantum computation requires the use of specially prepared ancillary quantum states called \textit{magic states}.

While the range of quantum applications is growing, an important class of applications is quantum simulation and quantum chemistry. These applications can not only take advantage of far horizon large-scale quantum computers, performing large-scale molecular simulation with applications in materials sciences and pharmaceuticals research, but they are indicative of a class of applications that will be able to take advantage of nearer-term 100-200 bit machines. This class of applications is especially dependent on specially prepared magic states.


Overall, this study attempts to develop a full scale estimate of realistic overheads and examine the tradeoffs present in the design of a dominating component of quantum computation. This tradeoff is between area and time: architectures can be designed that are small but impose large latency overheads, or larger amounts of area can be dedicated to resource production while simultaneously alleviating latency overhead. 
Figure~\ref{fig:tradeoffcartoon} illustrates the opposing trends for time and space as we factories are designed for higher rates of magic state production.  These two trends are  then combined into the space-time curve, with which a space-time optimal design points can be found.
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.75\linewidth]{Figures/tradeoffcartoon.png}
    \caption{Space and time tradeoffs exist for implementations of resource generation factories within quantum computers. By explicit overhead analysis, we can discover optimal space-time volume design points.}
    \label{fig:tradeoffcartoon}
\end{figure}

In summary, this paper makes the following contributions:
\begin{enumerate}[1.]
\item We quantify the time-space trade-offs in individual design decisions for magic state factories including the total number of factories and the total output states these factories can produce. 
\item We present a detailed study of different magic state distillation factory \textit{architectures}, and discover that distributed factory designs are space-time optimal.
\item We analyze the sensitivity of these optimal system configurations to fluctuations in underlying input parameter assumptions. We discover that time optimal design points suffer from significant performance degradation as the input parameters are allowed to fluctuate, while increasing the number of factories builds resilience into the system.
\end{enumerate}

The rest of the paper is structured as follows. In Section \ref{sec:bg}, a basic background of quantum computation, error correction, magic state distillation and the low-overhead Bravyi-Haah distillation protocol, as well as the Block Code state distillation construction. Section \ref{sec:related} describes previous work in this area. Section \ref{sec:motivate} discusses important characteristics of state distillation methods, and derives and highlights significant scaling behaviors that greatly impact full system overhead analysis. Section \ref{sec:model} describes in detail how these characteristics interact, and shows how these interactions create a design space with localized optimal points. Additionally, this section details our proposed multi-factory architectural design, and describes a procedure for discovering the optimal design points. Section \ref{sec:results} shows the impact of optimizing these designs, and examines the tradeoffs present within many different design points. 


==> old/model.tex <==
\section{Factory Latency Overhead}\label{sec:model}
 This section presents a systematic study of the resource-optimal architecture designs for realizing magic state distillation protocols. In particular, area and latency tradeoffs with respect to the factory architecture parameters $K$, $X$ and $\ell$ are described.

\subsection{Program Distributions}\label{subsec:program}

While the majority of the prior works on this subject have been abstracting algorithm behavior into a single number, the T gate count, we argue that the distribution of T-parallelism of a algorithm has a significant impact on the performance of the magic state factory.

Two Quantum chemistry algorithms would represent the two extremes of this parallelism feature. On one hand, the {\it Ground State Estimation} algorithm is one of those programs with very low T gate parallelism. An algorithm attempting to find the ground state energy of a molecule of size $m$, this application can be characterized by a series of rotations on single qubits \cite{whitfield2011simulation}. {\it Ising model}, on the other hand, is a highly parallel application demanding T gate at a much higher rate. This application simulates the interaction of an Ising spin chain, and therefore requires many parallelized operations across qubits, along with nearest neighbor qubit interactions \cite{barends2016digitized}. To capture application characteristics, we use the ScaffCC compiler toolchain that supports application synthesis from high-level quantum algorithm to to physical qubit layouts and circuits \cite{scaffcc}. 

The majority of the time steps in Ising Model algorithm has a large number of parallel T gates with a mean T load of 440, where as Ground State Estimation has no more than 12 T gates at each time steps. As opposed to just using the single T gate count to characterize algorithms, we will from now on use the distribution of T load. 

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{Figures/isinglatencies.pdf}
        \caption{Ising Model}
        \label{fig:time_is}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{Figures/gselatencies.pdf}
        \caption{Ground State Estimation}
        \label{fig:time_gse}
    \end{subfigure}
    \caption{Total number of surface code cycles required by two applications. Each figure is plotted for three different factory block-code levels $L=1,2,3$.}
    \label{fig:fact_time}
\end{figure*}

\subsubsection{T-Gate Contention and Congestion}\label{subsubsec:contentioncongestion}
In order to fully assess the space-time volume overhead of the system, we require a low level description of how the produced magic states are being consumed by the program. 

As discussed in the Section \ref{sec:bg}, a T gate requires braiding between the magic state qubit in the factory and the target qubit that the T gate operates on. Now suppose our factory is able to produce $K$ high-fidelity magic states per distillation cycle, and at some time step the program requests for $t$ T gates. If we demand more than the factory could offer at once (i.e. $t > K$), then naturally only $K$ of those requests can be served, while the others would have to wait for at least another distillation cycle. So we will say that the network has {\it contention} when the demand exceeds the supply capacity. By contrast, we define network {\it congestion} to capture the latency introduced by the fact the some braids may fail to route from the target to the factory on the 2D surface code layout, due to high traffic on this mesh network.

To estimate the overhead of network congestion, we will perform average case analysis without committing to a particular routing algorithm. Ideally, in the contention free limit where the number of requests $t$ is less than $K$, all requests could be scheduled and executed in parallel. However, often times the requests will congest due to limitations of routing algorithms. We define a congestion \textit{factor} $C_g$that represents the total latency required to execute all of the $T$ gate requests at any given time. 

We derive this congestion factor that scales proportional to the number of $t$ requests made at any given time, within a particular region serviced by a factory. This assumes a general topology, wherein a factory is placed in the center of that region, and all of the surrounding data qubits are served by this factory. Naturally, the center of the region is therefore quite dense with $T$ gate request routes. In general, for a reasonable routing algorithm, the number of routing options increases as area available increases. However, because all of the routes have their destination in the center of the region, increasing area of the region has no effect. In fact, the \textit{distance} of a $T$ request source from the factory increases the likelihood of congestion from a simple probabilistic argument. There may be other $T$ requests blocking available routes, and the number of these possible requests that block pathways increases as the distance between a request and the factory increases. The combination of these effects interacts with the complexity of a routing algorithm, and results in a scaling relationship proportional to both the $T$ request density $t$ and the maximum distance of any $T$ request within any of these regions:
\begin{align}
    C_g \sim c\sqrt{t} 
\end{align}
for some constant $c$, depending upon the routing algorithm.

\subsubsection{Latency Analysis}
Before we discuss further the two types of latency in detail, let's first consider some of the assumptions and implications of the general behaviors we observe.

We will assume throughout that the factory will keep producing $K$ states every distillation cycle $T_{distill}$, as in Equation \ref{eq:distilltime}. Of course we need to leave enough time for the T gate operations to finish (which takes about $T_t$ as in \ref{eq:tgatetime}) before we can restart the distillation procedure unless we buffer the produced magic states outside of the factory. However, both of these will have constant factor expanded in the volume that should affect all the design points equally. 

Observe in Figure \ref{fig:fact_time} that the total number of surface code cycles of state distillation decreases as the number of output capacity $K$ grows, simply because we are able to serve more magic states per distillation iteration. Notice that for high $K$, the trends converges to a constant, at which point increasing the capacity $K$ would no longer help reducing time because the factory is producing more states than needed by the program and will not be utilized. This can also be observed by comparing the plateau points of Figure \ref{fig:time_is} and \ref{fig:time_gse}, where parallel applications like Ising Model have higher T load width on average, so the convergence occurs at higher value of $K$. 

As keen readers may have already observed, for fixed output capacity $K$, it costs us both in time latency and in factory footprint to implement a high $\ell$ block-code factory, as shown in Figure \ref{fig:fact_time} and Figure \ref{fig:area_law}. The only reason we go after high $\ell$ is to achieve the desired target error rate. This relation is best captured in the bottom half of Figure \ref{fig:errorfeasible}, where the $L=1$ factory is not feasible for $K\ge 1$ since its output error rate is higher than the target error rate, while the $L=2$ factory is feasible for $K \in [1,50]$, and the $L=3$ factory is feasible for the entire plotted range.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.7\linewidth]{Figures/fullsuperimposedplot.png}
    \caption{Spacetime volume minimization under error threshold constraints imposed by target error rate for each block code level. An application will set a target error rate (black) that the factory must be able to achieve in output state fidelity. On the lower plot, levels 2 and 3 are the only levels available that can satisfy this. Moving to the upper plot, we find that the lowest volume in the feasible area is located on the level 2 factory.}
    \label{fig:errorfeasible}
\end{figure}

Since the distillation factory is always online and producing magic states, the overall time overhead is equal to the number of distillation iterations required to execute all the scheduled $T$ gate requests, multiplied by the time taken to distill one iteration $T_{\text{distill}}$ from Equation \ref{eq:distilltime}.

For any given program, characterized as a distribution $D$ of the T load, we denote $D[t]$ the number of timesteps in the program that $t$ parallel $T$ gates are to be executed. Then the number of iterations that the factory needs to distill to serve the $t$ requests can be computed based on the following latency analysis. In particular, in order to maximize the utilization of the factory, we would execute as many outstanding $T$ gate requests as possible in parallel. When the number of requests $t$ exceeds the factory yield $K$, we will need to stall the surpassed amount of requests. We denote $s = \lfloor t/K \rfloor$ the number of fully-utilized iterations. So, we are serving at full capacity for $s$ number of times, and at each time a congestion factor is being multiplied, as discussed in Section \ref{subsubsec:contentioncongestion}. It follows that the first $sK$ requests are completed in $s \sqrt{K}$ number of distillation cycles. And finally the rest $(t-sK)$ outstanding requests are then being executed in $\sqrt{t-sK}$ cycles. Notice that the last $(t-sK)$ requests could potentially be executed simultaneously with the T gate requests from the next time step, even when there exists explicit data dependencies between the left-over requests and new-coming ones. This is because the time it takes to execute the T gate is typically shorter than the factory distillation cycle time. So under the buffer assumption made earlier, we can stage the execution of requests within a distillation cycle such that no data dependencies are violated, as long as there are magic states available in the factory. We can have at most $T_{\text{distill}}/T_{\text{t}} \equiv 1/r$ stages. Therefore
\begin{align}
    n_{\text{distill}} = s \cdot \sqrt{\frac{K}{X}} + r \cdot \sqrt{\frac{t-sK}{X}}
\end{align}
where $K$ is again the yield of each iteration from Equation \ref{eq:koutput}.

Putting it together, we obtain our final time overhead of a factory:
\begin{align}
    T &= T_{\text{distill}} \cdot \Big(\sum_{t = 0}^{T_{\text{peak}}} n_{\text{distill}}\cdot D[t]\big)
\end{align}
where $T_{\text{peak}}$ is the maximum number of parallel T gates scheduled at one timestep.


\section{Area and Latency Tradeoffs}\label{sec:distributed}
\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{Figures/xtradeoffs.pdf}
    \caption{Space and time tradeoffs present by varying the distribution intensity of a factory architecture with a fixed capacity and number of levels.}
    \label{fig:xtradeoffs}
\end{figure}



While some distillation protocols offer no asymmetry to exploit, the Bravyi-Haah protocol in fact shows an area \textit{expansion} when a single factory is divided into many factories. Figure \ref{fig:xtradeoffs} illustrates this trend, where the $X$ corresponds to the lowest total area when it is set to 1. This arises from the original area law equation \ref{eq:arealaw}.

While dividing a single factory into many factories has a negative area impact, it also has many positive impacts that can serve to outweigh the drawbacks in certain scenarios. One such advantage is that for a fixed output capacity $K$, incrementing the number of factories used to produce that $K$ allows for all of those $K$ states to be provided at a much higher fidelity. The output error rate scales inversely with the number of factories on the lattice for a fixed output capacity $K$ as seen in Equation \ref{eq:errorround}.

This provides these architectures with the unique ability to actually manipulate the underlying \textit{physical error rate threshold}. In particular, substitution of $\frac{K}{X}$ for $K$ in all of the previous equations shows that the yield threshold now also has inverse dependence upon the number of factories used.

As Figure \ref{fig:xsweeperrorthresh} shows, for a fixed output capacity and block code level $\ell$, increasing the number of factories on the lattice can greatly increase the tolerable physical error rate under which the factory architecture can operate. 

With this knowledge, we are immediately presented with architectural tradeoffs. Using the representation of programs as distributions of $T$ gate requests, any application can be characterized by a $T_{\text{peak}}$, again defined as the highest number of parallel $T$ gate requests in any timestep of an application. For a time-optimal configuration, a system may set the factory output rate $K = T_{\text{peak}}$, so as to never incur any latency during the program execution. However, as the threshold in equation \ref{eq:thresh} indicates, this sets an upper bound on the tolerable input error rate $\epsilon_{\text{in}}$. With a distributed factory architecture, this provides a system parameter enabling systems to be designed that will be able to tolerate higher error rates, and still achieve the same output capacity $K$, at the expense of area as seen in the area law relationship from Figure \ref{fig:xtradeoffs}. Conversely, systems that are constructed with great knowledge of low underlying physical error rates may be able to reduce overall area of a time-optimal factory configuration by reducing the number of individual factories to a certain point. These are the tradeoffs in the design space that this work explores, and in fact we can find for representative benchmarks, configurations that are non-optimal in time that can save orders of magnitude in space-time overhead overall.  

As can be seen by comparing these plots, the space-time tradeoff favors the Mesh embedding technique. Throughout the rest of our analysis we restrict our focus to this layout, and devise analytical estimates justifed by simulation to model these overheads.

\subsection{Optimization Algorithm}\label{subsec:algo}
We combine all of the details of the explicit overhead estimation derived above in order to find optimal design points in the system configuration space. To do this, care must be taken to ensure that designs are capable of producing the target logical error rate for an application. Additionally, there exists a set of constraints $C$ that $K,X \in \mathbb{Z^+}$ have to satisfy: (i) $1 \le X \le K$; (ii) $K/X \le (1-8\epsilon_{\text{inject}})/(3\epsilon_{\text{inject}})$, due the Bravyi-Haah protocol error thresholds. With the feasible space mapped out, standard nonlinear optimization techniques are employed to explore the space and select the space-time optimal design point. 

With these constraints in mind, we explore the space by first selecting the lowest $\ell$ possible. As the area law and full volume scaling trends of the previous sections indicate, if there are any feasible design points with $\ell = \ell_0$, then any feasible design points for systems with $\ell_i > \ell_0$ will be strictly greater in overall volume. This is somewhat intuitive, as concatenation of block code protocols is very costly.

With the lowest $\ell$ selected, we check to see if there exists any feasible design points for this $\ell$ by solving the equation:
\begin{align}
    (1+3k^{\frac{1}{\ell}})^{2^{\ell}-1}\epsilon_{\text{inject}}^{2^{\ell}} \leq \frac{P_s}{N_{\text{gates}}}
\end{align}
If the $K$ that solves this equation is greater than or equal to 1, then there does exist feasible design space along this $\ell$, and the algorithm continues. Otherwise, $\ell$ is incremented. This iterative approach is used as an analytic solution of the above equation was not able to be found.

Next, nonlinear optimization techniques are used to search within the mapped feasible space for optimal design points in both $K$ and $X$. 

\begin{algorithm}
		\caption{Spacetime Optimization Procedure}
		\label{alg:opt}
		\algorithmicrequire{\;$P_s$, $N_{\text{gates}}$, $\epsilon_{\text{inject}}$, distribution $D$ and constraints $C$}
		
		\algorithmicensure{\; $K$, $X$}
		\begin{algorithmic}[1]
		\Procedure{Optimize}{}
		    \State $K \gets 1$, $X \gets 1$, $\ell_{\text{max}} = 5$
		    \State $\epsilon_{\text{target}} \gets P_s/N_{\text{gates}}$
			\For{$\ell \in [1,\ell_{\text{max}}]$}
			\State $k_\ell \gets (K/X)^{1/\ell}$
			\State $n_\ell \gets 3k_\ell + 8$
			\For{$r \in \{1, \cdots \ell\}$}
			    \If{$r==\ell$} $\epsilon_r \gets \epsilon_{\text{target}}$
			    \Else \;$\epsilon_r \gets (1+3k_\ell)^{2^r-1}\epsilon_{\text{inject}}^{2^r}$
			    \EndIf
			    \State $d_r \gets \text{Solve}\{d_r \cdot (100 \epsilon_{\text{in}})^{(d_r+1)/2} = \epsilon_r, \; d_r\}$
			\EndFor
			
				\State $R\equiv K/X \gets \text{Solve}\{\epsilon_{\ell} = \epsilon_{target},\;R\}$
				\If {$R \geq 1$}
				    \State $K_{\text{output}}\gets K \cdot \prod_{r=1}^{\ell}\big[(1-n_\ell\cdot\epsilon_{\text{inject}})\epsilon_r\big]$
				    \State $s \gets \lfloor t/K_{\text{output}}\rfloor$
				    \State $T_{\text{t}} \gets 4d_\ell + 4$
				    \State $T_{\text{distill}} \gets 11\sum_{r=1}^\ell d_r$
				    \State $n_{\text{distill}} \gets s\cdot \sqrt{\frac{K_{\text{output}}}{X}} + T_t/T_{\text{distill}}\cdot\sqrt{\frac{t-sK_{\text{output}}}{X}}$
				    \State $T_{\text{total}} \gets T_{\text{distill}}\Big(\sum_{t=0}^{T_{\text{peak}}}n_{\text{distill}}\Big)\cdot D[t]$
				    \State $A_{\text{factories}} \gets X\cdot n_l^{\ell-1}\cdot(6k_\ell + 14)\cdot d_1^2$ 
				    \State $(K,X)$ \gets \;$\argmin_{(K,X):C}\; A_{\text{factories}} \cdot T_{\text{total}}$
				\Else
				    \State $\ell \gets \ell + 1$
				\EndIf
			\EndFor
			\State \Return $K,X$
		\EndProcedure
		\end{algorithmic}
	\end{algorithm}


==> old/motivation.tex <==
\section{Factory Area Overhead}\label{sec:motivate}

\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[trim=0 0 0 0,
        width=\textwidth]{Figures/xsweepoutputerrs.pdf}
        \caption{Error rate attainable by number of factories.}
        \label{fig:yield}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.23\textwidth}
    \includegraphics[width=\linewidth]{Figures/xsweeperrorthreshold.pdf}
    \caption{Physical error rate tolerable by number of factories}
    \label{fig:xsweeperrorthresh}
    \end{subfigure}    \caption{(a)Higher fidelity output states are achievable with increasing number of factories at a fixed output capacity. (b) Increasing the number of factories in an architecture allows for higher tolerance of input physical error rates}
    \label{fig:factorieserrorsyields}
\end{figure}
A magic state distillation factory architecture can be characterized by three parameters: total magic state output capacity $K$, number of factories on the lattice $X$, and block code level $\ell$. For simplicity, we assume uniform designs where all $K$ output states are to be divided equally into $X$ factories, all of which operate at level $\ell$. We now analyze the constructs presented in Section \ref{sec:bg} to derive full magic state factory scaling behaviors with respect to these architectural design variables. As we will see, these behaviors interact non-trivially, and lead to space-time resource consumption functions that show optimal design points. 

First we examine the fidelity of output magic states that is attainable for a given factory configuration, along with expected number of states that will in fact be made available. Applying the block code error scaling relationship, as the number of levels of a magic state factory increases, the output error rates attainable scale double-exponentially with $\ell$. In fact, for a given round $r$ of a factory, the explicit form of the output error rate can be written as:
\begin{align}
\epsilon_r &= (1+3(K/X)^{\frac{1}{\ell}})^{2^r-1}\epsilon_{\text{inject}}^{2^r}\label{eq:errorround}
\end{align}
where $(K/X)$ denotes the size of each factory on a lattice. 

The yield rate of a particular factory can be expressed as a function involving the error rate attained after round $r$ of distillation has been performed:
\begin{align}
K_{\text{output}} &= K \cdot \prod_{r=1}^{\ell}\bigg[(1-(3(K/X)^{\frac{1}{\ell}}+8)\epsilon_{r-1}\bigg]\label{eq:koutput}
\end{align}

Equation \ref{eq:koutput} actually imposes a \textit{yield threshold} on the system, where for a given $K$ and $\ell$, a system will have a vanishing success probability as the injected physical error rate increases. This threshold can be seen by examining the product term, and noting that yield must be positive to be able to compensate for lossy factory behavior with repetition. Hence, the leading term requires: $1-(3(K/X)^{1/\ell} + 8)\epsilon_{\text{inject}} > 0$, and thus:

\begin{align}
    \epsilon_{\text{thresh}} \approx \frac{1}{3(K/X)^{1/\ell}+8}\label{eq:yieldthresh}
\end{align}

Notice that as higher levels $\ell$ are built into the factory, the location of the yield dropoff point in terms of the specified output state capacity $k$ occurs at higher and higher sizes. This behavior will be useful when we analyze full quantum applications, as the yield behavior must balance with application demand for magic states.

(a) shows the yield rate scaling behavior of factories of block-code levels $L=1,2,3$ with fixed $X=1$. Large factories can produce many more states, but this comes at the cost of a reduction in overall state fidelity achievable, and potentially a yield penalty. Any given factory has a particular drop-off capacity $K$ for which the expected number of produced states becomes vanishingly small. Higher levels increase the location of this threshold point. 

\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[trim=0 0 0 0,
        width=\textwidth]{Figures/factoryyieldbyblocklevel.pdf}
        \caption{Factory yield rate by block level.}
        \label{fig:yield}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\linewidth]{Figures/area_law.pdf}
        \caption{Area scaling by factory round}
        \label{fig:area_law}
    \end{subfigure}
    \caption{(a) Increasing factory output capacity puts pressure on the factory yield rate, and increasing the number of levels pushes the yield dropoff point. (b) Maximum area to support multi-level factory is required of the lowest level of the factory, all higher levels require less area support.}
    \label{fig:factorycharacteristics}
\end{figure}


    
\subsection{Full Area Costs}
Plugging in the specific values of the Bravyi-Haah protocol to the area scaling relationship derived above will allow us to explicitly describe 
which is shown graphically on Figure \ref{fig:area_law}.

Importantly, we find that for all $\ell$ level factories with $\ell \geq 1$, the area of the first round exceeds the area required for all other rounds. We arrive at
the area in terms of physical qubits of a factory architecture specified by $K$, $X$, and $\ell$ as:
\begin{align}
   A_r&=X\cdot(K/X)^{\frac{r-1}{\ell}}\big[3(K/X)^{\frac{1}{\ell}}+8\big]^{\ell-r}\big[6(K/X)^{\frac{1}{\ell}}+14\big]\cdot d_r^2 \label{eq:arealaw}\\
   &\le X\big[3(K/X)^{\frac{1}{\ell}}+8\big]^{\ell-1}\big[6(K/X)^{\frac{1}{\ell}}+14\big]\cdot d_1^2
\end{align}
In an aggressively optimized factory design then, one could conceivably save space within the distillation procedure by utilizing the space differential between successive rounds of distillation for other computation. For simplicity, and for ease of classical compilation of the quantum circuitry, we will assume that this cannot be done. Instead, the first round area of any given factory \textit{defines} the area required by that factory, over the length of its entire operation. As a result, Figure \ref{fig:area_k} describes the scaling of factory area both by successive $\ell$ and by increasing output capacity $K$. 

\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{Figures/xareascaling.pdf}
        \caption{Area required to implement a 2-level factory of varying distribution densities $X$. As the distribution intensity approaches full distribution where $X = K$, the total area increases significantly faster as factory output is scaled up.}
        \label{fig:area_k}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[trim=0 0.2in 0 0, width=\textwidth]{Figures/xlatencies.pdf}
       \caption{Latency as it scales with factory output capacity. For factories of a fixed size, increasing the number of factories on the lattice reduces latency overall and will speed up application execution time. This comes from reductions both in contention and congestion of the factory network.}
      \label{fig:time_k}
    \end{subfigure}
    ~
        \caption{Space and Time Required by Block-Code Levels $L=1,2,3$.{Higher $K$ factories can produce states slightly faster than low $K$  factories, due to a limitation on the output error rate.}}
    \label{fig:factoriesspacetime}
\end{figure*}        


==> old/old_related.tex <==
\section{Related work}\label{sec:related}
\begin{figure}[b]
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
    \includegraphics[width=\linewidth]{Figures/unifactories.png}
    \caption{Unified Factory Architecture Diagram}
    \label{fig:unifactory}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.23\textwidth}
    \includegraphics[width=\linewidth]{Figures/distfactories.png}
    \caption{Distributed Factory Architecture Diagram}
    \label{fig:distfactory}
    \end{subfigure}
    \caption{The concept of a unified versus distributed factory architecture, embedding factories within computational surface code region.}
    \label{fig:fact_time}
\end{figure}
Previous work on this subject has assumed either that magic states will be prepared offline in advance \cite{fowler2013surface}, or that the  production rate is set to keep up with the {\it peak} consumption rate in any given quantum application, and any excess states will be placed in a buffer \cite{campbell}. This paper focuses on the design of these magic state factories. It presents a detailed model of the space and time costs of design decisions involved in magic state factory design, allowing for a realistic comparison of several potential designs. To this end, this work assumes that magic state factories will be active during the computation, and states will not be able to be prepared offline or in advance. This work quantifies the time penalty imposed if no states are available and computation must wait for a magic state factory to prepare the state.

Prior work also analyzed the overhead of CNOT operations which dominate other classes of applications like quantum cryptography and search optimization \cite{javadi2017optimized}. For this paper we focus on quantum chemistry and simulation applications that are likely to represent a large proportion of quantum workloads. 


==> old/old_results.tex <==
\section{Results}\label{sec:results}
The overhead of various factory architectures is examined and compared across a set of representative quantum chemistry and simulation workloads. Specifically, we examine the full program behavior of both Ising Model simulation and Ground State Estimation of a molecule of small size. As these are the two applications that have been implemented in the ScaffCC end-to-end compiler framework, we performed a detailed analysis of their program behavior and how it interacts with factory architectures. We sweep over input problem sizes and discover that these architectures behave fairly regularly across varying program widths for these applications. Additionally, as quantum chemistry and simulation applications are fairly predictable in structure as described in Section \ref{sec:bg}, the Ising Model and Ground State Estimation algorithm are representive benchmarks of this space.

A comparison is made in Figure \ref{fig:timespaceoptimal} between the time optimal configuration and the space optimal configuration, both unified designs. This comparison represents the range between two ends of the design space spectrum, and each shows a particular error rate range over which it performs more optimally. Initially, at the highest input error rate, the space optimal design requires more resources than the time optimal design, as the application suffers from excessive latency from magic state factory access time. Note the inflection points at $10^{-3.5}$ and $10^{-4.5}$ input error rates. At this point, the space optimal factory is able to reduce the $\ell$ block code distillation level as input error rates are sufficiently high. This reduction in area compensates over this region against the expansion in computation time, and the design is about to outperform the time optimal configuration. At $10^{-4.5}$, this occurs for the time optimal design, and the space correction once again enables the time optimal design to outperform the other.
\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{Figures/timespaceoptimal.pdf}
    \caption{Comparing time and space optimal designs. There are regions where each outperforms the other, showing great sensitivity to the underlying physical error rate the the corresponding required $\ell$ level.}
    \label{fig:timespaceoptimal}
\end{figure}

\begin{figure}[b]
    \centering
    \begin{subfigure}[b]{0.45\linewidth}
    \includegraphics[width=\linewidth]{Figures/ising500results.pdf}
    \caption{Ising Model}
    \label{fig:isingresults}
    \end{subfigure}
    \begin{subfigure}[b]{0.45\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/gseresults.pdf}
    \caption{Ground State Estimation}
    \label{fig:gseresults}
    \end{subfigure}
    \caption{Spacetime volume reductions of fully optimized designs over time optimal designs for both Ising Model and Ground State Estimation. While Ising Model is intrinsically more parallel which leads to high choices of output capacity, both applications still show between a 12x and 16x reduction in overall spacetime volume.}
    \label{fig:appresults}
\end{figure}

Figures \ref{fig:isingresults} and \ref{fig:gseresults} depict the detailed results of our optimization procedure on the Ground State Estimation and Ising Model applications. Ising Model is intrinsically very parallel, which leads to a higher optimal capacity choice for the fully optimized factory, however it is able to choose a distribution level that saves approximately 15x in spacetime volume. Ground State Estimation is very serial, yet for sufficiently low error rates the optimized design is able to incorporate distribution of factories into the lattice to lower the required block code concatenation level $\ell$, resulting in a 12x reduction in volume across these points.

Figure \ref{fig:fullvols} depicts the full spacetime volume required by different factory architectures across the design space. Shown are four configurations: a time optimal unified factory configured with output capacity $K = T_{peak}$, a space optimal unified factory with $K=1$ an optimal capacity unified factory, and an optimal capacity optimally distributed factory. 

Distinct volume phases are evident visually on the graph. Sweeping from high error rates to low error rates, large volume jumps occur as observed before, for specific configurations when that configuration can switch to a lower level of rounds of block code distillation in order to convert the input error rate to the target output error rate. Notice that this jump occurs earliest for the space-optimal, capacity-optimal, and distributed capacity-optimal designs, at $10^{-3.5}$ input error rate. All of these designs show an inflection point here, where a lower block code distillation level is required to achieve the output error rate. This is not true of the time optimal factory, which in fact has the largest output capacity of the set. Because the output capacity is so high, the lowest achievable output error rate is much higher than that of the other designs. This forces the block code level to remain high until the input error rate becomes sufficiently low, which occurs at $10^{-4.5}$. 

As Figure \ref{fig:spacereduction} describes, the optimized distributed factory architecture is able to save between 1.2x and 4x in total space-time volume over the optimized unified factory. Large volume jumps occur primarily between $10^{-3.5}$ and $10^{-3.4}$ physical error rate, and this again corresponds to a requirement by this application to increment to a higher block code level $\ell$, which happens for both the unified and distributed factory schemes. 
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.45\linewidth}
    \includegraphics[width=\linewidth]{Figures/ising1000reductions.pdf}
    \caption{Ising Model N=1000}
    \label{fig:ising1000}
    \end{subfigure}
    \begin{subfigure}[b]{0.45\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/ising2000reductions.pdf}
    \caption{Ising Model N=2000}
    \label{fig:ising2000}
    \end{subfigure}
    \caption{Ising Model with varying problem sizes, comparing time optimal factories against fully space-time optimized configurations. We see that the trend of between 15x and 20x total volume reduction extends to larger molecular simulations.}
    \label{fig:spacetimeisingresults}
\end{figure}
Figures \ref{fig:ising1000} and \ref{fig:ising2000} detail these trends as larger and larger quantum simulation applications are executed. Even for extremely large simulations, we find that fully optimizing a factory design yields between a 15x and 18x full volume reduction, scaling with sensitivity to physical error rates that require designs to change block code distillation level. 

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.45\linewidth}
    \includegraphics[width=\linewidth]{Figures/space_reduction.pdf}
    \caption{Space Tradeoff}
    \label{fig:spacereduction}
    \end{subfigure}
    \begin{subfigure}[b]{0.45\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/time_reduction.pdf}
    \caption{Time Tradeoff}
    \label{fig:timereduction}
    \end{subfigure}
    \begin{subfigure}[b]{0.60\linewidth}
        \includegraphics[width=\linewidth]{Figures/kvalsising.pdf}
    \caption{Output Capacities Chosen by Optimized and Unified Factory Architectures}
    \label{fig:kvals}
    \end{subfigure}
    \caption{Spacetime volume reduces by moving from a capacity optimized factory to a fully optimized distributed factory, as the designs trade space for time. Magic state access latency is a dominating effect in these applications, as can be seen by the large capacity values chosen by the optimized factory configuration.}
    \label{fig:optimizedreductionresults}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/full_volume_reduction.png}
    \caption{Full volume comparison across distillation factory architectures.} 
    \label{fig:fullvols}
\end{figure}

As Figures \ref{fig:spacereduction} and \ref{fig:timereduction} indicate, these optimal volume designs trade space for time, and the net effect is an overall volume reduction, indicating that for these highly parallel quantum chemistry applications the magic state factory access latency is a much more dominating effect. 

Figure \ref{fig:kvals} depicts the output capacities discovered by the optimized factory architecture as well as the optimal capacity chosen for a unified architecture comprised of a single factory. Notably, at both ends of the input error rate spectrum we find that both factory architectures choose the same output capacity, as in the high error rate case this is driven by high $\ell$ requirement, while in the low error rate limit both factory architectures can afford to be very large and not suffer from any yield penalties. 


==> old/sensitivity.tex <==
\section{Sensitivity Analysis} \label{sec:sensitivity}
Supposing that a design choice has been made specifying the desired factory capacity $K$, number of factories $X$, and block code distillation level $\ell$, different design points show varying sensitivity to fluctuations in the underlying design points around which the architectures were constructed. For example, Figure \ref{fig:sens} details an instance of this occurrence. The figure shows three different designs: a time optimal design with $K$ set to the peak parallelism of the Ising Model application and $X=1$ for unification, a space optimal design with $K=X=1$ for the absolute minimum required space overhead, and a fully optimized design in this case setting $K\sim 600$ and $X \sim 200$. All of these factories were designed under the assumption that the physical machine will operate with $10^{-5}$ error rate, which is an optimistic assumption.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figures/error_sensitivity.pdf}
    \caption{Factory Architectures and Sensitivity to Fluctuations in Underlying Physical Error Rates}
    \label{fig:sens}
\end{figure}

Important to notice is that while these applications perform similarly over the range from $10^{-5}$ to $10^{-4}$, it is just after this point that the time optimal factory encounters a steep volume expansion. This is due to the underlying yield threshold equation \ref{eq:yieldthresh}. For this design the threshold of tolerable physical error rates is quite high, significantly higher than that of the other designs. Because of this, it can only tolerate a smaller range of fluctuation in the underlying error rate before it ceases to execute algorithms correctly.

==> old/simulation.tex <==
\section{Simulation and Validation}\label{sec:simulation}
This section explores the validity of our models through empirical evaluation of the spacetime resources. To do this, we use surface code simulation tools~\cite{javadi2017optimized} to accurately assess the latency and qubit cost of fully error-corrected applications with various magic state distillation factory configurations. Validation through simulation is especially important in applications with high parallelism (i.e. Ising Model), since the analytical model may not accurately capture issues of traffic and congestion. For serial applications (i.e. Ground State Estimation), 

Figure~\ref{} shows simulation results superimposed on top of those driven analytically. We see a close correspondence. This is due to two factors. First, our distributed factory architecture is good at avoiding congestion, because each qubit's magic state needs are served from the nearest port of the nearest factory, in a highly local manner. Secondly, for any remaining congestion, the braid simulation tool in~\cite{javadi2017optimized} employs various braid prioritization heuristics to avoid points of traffic. The end result is that our models can be verified against empirical evaluation of resources.

Using these simulations, we can also verify optimal operating points in the spacetime tradeoff spectrum. This is a concretization of Figure~\ref{fig:tradeoffcartoon}, and is depicted in Figure \ref{fig:meshtradeoff} for the Ising Model application. We see that as factory capacities increase, the applications time improves at the expense of its qubit numbers. In this figure, the spacetime volume is sketched in black, and has two near-optimal points: one with relatively few qubits but high latency, and vice versa. The worst performance occurs in the middle of this spectrum, when transition from level 1 to level 2 distillation needs to occur (causing a sudden jump in qubits, but not much latency improvement).

\begin{figure}[htb]
  \centering  
  \includegraphics[width=\columnwidth]{Figures/MagicTradeoffMesh.pdf}
  \caption{Spacetime tradeoff for varying factory capacities. Optimal spacetime volume (black dotted line) can be chosen in two places ($K\approx40$ and $K\approx750$), one corresponding to a low-qubit, high-latency configuration and the other vice versa.}
  \label{fig:meshtradeoff}
\end{figure}
